TaskWeb: Selecting Better Source Tasks for Multi-task NLP

Recent work in NLP has shown promising results in training models on large amounts of tasks to achieve better generalization. However, it is not well-understood how tasks are related, and how helpful training tasks can be chosen for a new task. In this work, we investigate whether knowing task relationships via pairwise task transfer improves choosing one or more source tasks that help to learn a new target task. We provide TaskWeb, a large-scale benchmark of pairwise task transfers for 22 NLP tasks using three different model types, sizes, and adaptation methods, spanning about 25,000 experiments. Then, we design a new method TaskShop based on our analysis of TaskWeb. TaskShop uses TaskWeb to estimate the benefit of using a source task for learning a new target task, and to choose a subset of helpful training tasks for multi-task training. Our method improves overall rankings and top-k precision of source tasks by 10% and 38%, respectively. We also use TaskShop to build much smaller multi-task training sets that improve zero-shot performances across 11 different target tasks by at least 4.3%.

==> sections_emnlp_final/acknowledgements.tex <==
% We thank members of the H2Lab and UW NLP for their discussion and constructive feedback. 
% This work was funded in part by the DARPA MCS program through NIWC Pacific (N66001-19-2-4031), NSF IIS-2044660, and gifts from AI2.
% Joongwon Kim is supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-2140004.
% Akari Asai is funded by the IBM PhD Fellowship. 

==> sections_emnlp_final/conclusion.tex <==
% In this work, we investigate how using prior knowledge of task relationships quantified via pairwise task transfer aids selecting helpful source tasks for multi-task NLP.
% We build \data, a benchmark and repository of pairwise task transfers across different tasks, models and adaptation methods in NLP.
% Based on our analysis of \data, we propose \algo, our method for selecting helpful source tasks for a new target task.
% We show that \algo outperforms existing methods in choosing helpful source tasks for different target tasks.
% Moreover, we use \algo and \data to build small multi-task training sets and outperform other methods that use much larger training sets.

==> sections_emnlp_final/limitations.tex <==
Our work contains several limitations.
First, our set of tasks does not constitute the entirety of NLP tasks.
While we use 22 NLP tasks that are representative enough to cover various types of reasoning, we do not include long-form tasks (e.g., summarization, LFQA) or domain-specific tasks (e.g., law, medicine) to facilitate experiments across various model architectures such as encoder-only models.
In order to add entirely new forms of task to \data, one would have to compute pairwise transfer scores between the new task and other tasks in \data. If the model is known beforehand, this would require $\|T\|$ iterations of fine-tuning with 1,000 examples where $T$ is the set of tasks in \data. On the other hand, if the model is not known beforehand, this would require $\|M\|\times\|T\|$ iterations where $M$ is the set of models used in \data.

Moreover, our datasets are in English and we do not incorporate multilinguality in our experiments.
% we note that real users often apply large language models to highly customized tasks that may or may not benefit from knowledge associated with tasks in \data.
Second, our work focuses on models with at most three billion parameters.
Our finding may not be directly applicable to models with orders of magnitude more parameters considering factors such as emergence \cite{DBLP:journals/tmlr/WeiTBRZBYBZMCHVLDF22}, which can be explored in future work.
Third, we perform our multi-task finetuning experiments by uniformly sampling 2,000 examples from each source task following the style of \citet{DBLP:conf/emnlp/WangMAKMNADASPK22}.
Therefore, different behavior may arise when other sampling strategies are used.
Finally, recent work shows the effectiveness of using diverse instruction-output pairs which do not necessarily have clear boundaries as our tasks do \cite{DBLP:conf/nips/Ouyang0JAWMZASR22, DBLP:journals/corr/abs-2212-10560, DBLP:journals/corr/abs-2306-04751}.
Recently, \citealt{DBLP:journals/corr/abs-2306-04751} report that large language models finetuned on specific instruction datasets perform better on related target tasks, which is closely related to our findings.
Future work could extend our approach to setups without clear boundaries between tasks and explore ways to perform target-specific instruction tuning.
Considering these limitations, we encourage the NLP community to contribute to quantifying the transferabilities between different language tasks.
